Iodine: Verifying Constant-Time Execution of Hardware

To be secure, cryptographic algorithms crucially rely on the underlying hardware to avoid inadvertent leakage of secrets through timing side channels. Unfortunately, such timing channels are ubiquitous in modern hardware, due to its labyrinthine fast-paths and optimizations. A promising way to avoid timing vulnerabilities is to devise --- and verify --- conditions under which a hardware design is free of timing variability, i.e., executes in constant-time. In this paper, we present Iodine: a clock precise, constant-time approach to eliminating timing side channels in hardware. Iodine succeeds in verifying various open source hardware designs in seconds and with little developer effort. Iodine also discovered two constant-time violations: one in a floating-point unit and another one in an RSA encryption module.

==> horn.tex <==



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> merge.tex <==
% \begin{figure}
%   \centering
%   \lstinputlisting[style={verilog-style}]{merging11.v}
%   \caption{Merging 1: Before merging}
%   \label{fig:merging01}
% \end{figure}

% \begin{figure}
%   \centering
%   \lstinputlisting[style={verilog-style}]{merging12.v}
%   \caption{Merging 1: After merging}
%   \label{fig:merging01}
% \end{figure}

% \begin{figure}
%   \centering
%   \lstinputlisting[style={verilog-style}]{merging21.v}
%   \caption{Merging 2: Before merging}
%   \label{fig:merging01}
% \end{figure}

% \begin{figure}
%   \centering
%   \lstinputlisting[style={verilog-style}]{merging22.v}
%   \caption{Merging 2: After merging}
%   \label{fig:merging01}
% \end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

